MULTITAT: Benchmarking Multilingual Table-and-Text Question Answering

Question answering on the hybrid context of tables and text (TATQA) is a critical task, with broad applications in data-intensive domains. However, existing TATQA datasets are limited to English, leading to several drawbacks: (i) They overlook the challenges of multilingual TAT-QA and cannot assess model performance in the multilingual setting. (ii) They do not reflect real-world scenarios where tables and texts frequently appear in non-English languages. To address the limitations, we propose the first multilingual TATQA dataset (MULTITAT). Specifically, we sample data from 3 mainstream TATQA datasets and translate it into 10 diverse languages. To align the model TATQA capabilities in English with other languages, we develop a baseline, Ours. Experimental results reveal that the performance on non-English data in MULTITAT drops by an average of 19.4% compared to English, proving the necessity of MULTITAT. We further analyze the reasons for this performance gap. Furthermore, Ours outperforms other baselines by an average of 3.3, demonstrating its effectiveness.

==> tab/basic_statistics.tex <==
\begin{tabular}{@{}lc@{}}
\toprule
%  & \# \\ 
% \midrule
Question       & $250$   \\
Hybrid Contexts & $233$   \\
Avg. Rows      & $10.2$  \\
Avg. Columns   & $4.7$   \\
Avg. Paragraphs & $5.3$   \\
\bottomrule
\end{tabular}

==> tab/error.tex <==
\begin{tabular}{llc}
\toprule
\textbf{Error Type} & \textbf{Description} & \textbf{Proportion} \\
\midrule
Linking & Associating entities in the question with incorrect information in tables or text & $48$   \\
Formula & Uses an incorrect formula, resulting in erroneous output & $24$  \\
Redundancy & Outputting irrelevant information beyond the correct answer & $24$  \\
Other &- & $4$\\
\bottomrule
\end{tabular}
